Light Field Implicit Representation for Flexible Resolution Reconstruction

Inspired by the recent advances in implicitly representing signals with trained neural networks, we aim to learn a continuous representation for narrow-baseline 4D light fields. We propose an implicit representation model for 4D light fields which is conditioned on a sparse set of input views. Our model is trained to output the light field values for a continuous range of query spatio-angular coordinates. Given a sparse set of input views, our scheme can super-resolve the input in both spatial and angular domains by flexible factors. consists of a feature extractor and a decoder which are trained on a dataset of light field patches. The feature extractor captures per-pixel features from the input views. These features can be resized to a desired spatial resolution and fed to the decoder along with the query coordinates. This formulation enables us to reconstruct light field views at any desired spatial and angular resolution. Additionally, our network can handle scenarios in which input views are either of low-resolution or with missing pixels. Experiments show that our method achieves state-of-the-art performance for the task of view synthesis while being computationally fast.

==> ablation_networkparam.tex <==
    \begin{table}[h]
        
        \centering
\begin{tabular}{llll}
\hline
$h$ &$d$& $d_{MLP}$ & PSNR/SSIM\\
\hline
2&160&320&42.80/0.986\\
2&180&350&42.76/0.986\\
2&128&256&42.67/0.985\\
2&128&192&42.53/0.985\\
3&160&320&42.72/0.986\\
3&128&192&42.53/0.985\\
\hline
\end{tabular}
        \caption{Quantitative comparisons (PSNR/SSIM) of CILN trained for $7\times7$ view interpolation with different network parameters on 30 scenes test set. In the table, $h$ indcates number of hidden layers in MLP, $d$ indicates per pixel feature dimension, and $d_{MLP}$ indicates hidden layer dimension of the implicit network.\label{tab:ablation_net_param}}
        \end{table}


==> table_missing_pixels.tex <==
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llrrr}
\hline
p                     & Method     & 30scenes       & Occlusions     & Reflective \\ \hline
\multirow{4}{*}{0.00} & Meng~et~al.\cite{meng2019high}  &40.18/0.975&36.69/0.969&37.59/ 0.952\\
                      & Wu~et~al.\cite{wuTIP2019} & 39.27/0.976            & 34.43/0.956            & 36.46 /0.947          \\
                      & Ours       &42.34/0.985&38.83/0.979&38.89/0.960 \\ 
                      & Ours-clean&\textbf{42.80/0.986}&\textbf{39.36/0.981}&\textbf{39.13/0.960}\\\hline
\multirow{4}{*}{0.25} & Meng~et~al.\cite{meng2019high}\textsuperscript{*} &38.67/0.972 &35.88/0.964&36.67/0.948\\
                      & Wu~et~al.\cite{wuTIP2019}\textsuperscript{*}  & 37.82/0.970          & 33.74/0.949           & 35.48/0.942 \\
                      & Ours       &41.90/0.983&38.41/0.978 & 38.51/0.959\\
                      \hline
\multirow{4}{*}{0.50} & Meng~et~al.\cite{meng2019high}\textsuperscript{*}   & 37.73/0.963&34.66/0.951&35.79/0.938
\\
                      & Wu~et~al.\cite{wuTIP2019}\textsuperscript{*} & 36.84/0.961          & 32.76/0.934            & 34.67/0.931 \\
                      & Ours       &41.02/0.980&37.54/0.973&37.86/0.954\\ \hline
\multirow{4}{*}{0.75} & Meng~et~al.\cite{meng2019high}\textsuperscript{*}  & 34.85/0.933&31.83/0.904& 33.37/0.906\\
                      & Wu~et~al.\cite{wuTIP2019}\textsuperscript{*} & 34.15/0.929          & 30.45/0.885            & 32.47/0.901          \\
                      & Ours       & 38.76/0.970 & 35.33/0.958&36.33/0.942\\ \hline
\multirow{4}{*}{0.90} & Meng~et~al.\cite{meng2019high}\textsuperscript{*}   & 30.77/0.864&27.88/0.796&30.03/0.848 \\
                      & Wu~et~al.\cite{wuTIP2019}\textsuperscript{*} & 30.39/0.863          & 27.21/0.788          & 29.42/0.845          \\
                      & Ours       &34.59/0.934  &31.41/0.907  &33.23/0.908               \\ \hline
\end{tabular}}
\caption{Average PSNR of novel views in dB for $7\times7$ view synthesis. p indicates the fraction of missing pixels. $*$ indicates the results of \cite{wuTIP2019,meng2019high} with restored inputs. %$**$ indicates the results of 4D-Conv approach of~\cite{meng2019high} retrained on input views with sparse pixels. 
Our CILN is trained on varying number of missing pixels 0-90\%.}
\label{tab:missing}
\end{table}
